SREGym: A Live Benchmark for AI SRE Agents with High-Fidelity Failure Scenarios

AI agents are increasingly used to diagnose and mitigate failures in production systems, known as agentic Site Reliability Engineering (SRE). Current SRE benchmarks are limited to oversimplistic SRE tasks and are unfortunately hard to extend due to bespoke designs. We present SREGym, a high-fidelity benchmark for SRE agents. SREGym exposes a live system environment built atop real-world cloud-native system stacks, where high-fidelity failure scenarios are simulated through fault injectors. SREGym models the complexity of production environments by simulating (1) a wide range of faults at different layers, (2) various ambient noises, and (3) diverse failure modes such as metastable failures and correlated failures. SREGym is architected as a modular, extensible framework that orchestrates fault and noise injectors across stacks. SREGym currently includes 90 realistic, challenging SRE problems. We use SREGym to evaluate frontier agents and show that their capabilities varies significantly in addressing different kinds of failures, with up to 40% differences in end-to-end results. SREGym is actively maintained as an open-source project and has been used by researchers and practitioners.

==> figs/fig-faults.tex <==
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.35\textwidth}
        \centering
        \includegraphics[width=1.05\textwidth]{figs/bad_sector.pdf}
        \vspace{-5pt}
        \caption{Bad sectors in hard disk drives}
        \label{fig:latent-sector-error}
    \end{subfigure}
    \hspace{0.01\textwidth}
    \begin{subfigure}[t]{0.295\textwidth}
        \centering
        \includegraphics[width=1.05\textwidth]{figs/metastable.pdf}
        \vspace{-5pt}
        \caption{Metastable behavior}
        \label{fig:metastable-fault}
    \end{subfigure}
    \hspace{0.01\textwidth}
    \begin{subfigure}[t]{0.315\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figs/concurrent.pdf}
        \vspace{-5pt}
        \caption{Concurrent failures}
        \label{fig:noisy-environment}
    \end{subfigure}
%    \vspace{-5pt}
    \caption{The \bench{} problems we will use in the demonstration where the Stratus SRE agent will be applied 
        to tackle them. The problems, as well as the SRE agent behavior, are described in \S\ref{sec:agent}.
        The service graphs are simplified for clarity.}
    \label{fig:failures}
\end{figure*}


==> figs/tab-conditional-mit.tex <==
\begin{wraptable}{r}{0.5\textwidth}
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{llcc}
        \toprule
        Agent & Noise & $P(\text{M} \mid \text{D✓})$ & $P(\text{M} \mid \text{D✗})$ \\
        \midrule
        Stratus \claude{}  & ✗ & 0.892 & 0.615 \\
        Stratus \claude{}  & ✓  & 0.770 & 0.443 \\
        Stratus \kimi{}   & ✗ & 0.679 & 0.217 \\
        Stratus \kimi{}   & ✓  & 0.699 & 0.246 \\
        Claude Code          & ✗ & 0.836 & 0.541 \\
        Claude Code          & ✓  & 0.858 & 0.604 \\
        Codex                & ✗ & 0.762 & 0.346 \\
        Codex                & ✓  & 0.775 & 0.391 \\
        \bottomrule
    \end{tabular}
    \caption{Conditional probability of successful mitigation (\textbf{M})
        given diagnosis (\textbf{D}) outcome.
        % Higher $P(\text{Mit} \mid \text{Diag}\checkmark)$ indicates
        % stronger execution given correct understanding;
        % higher $P(\text{Mit} \mid \text{Diag}\times)$ indicates
        % mitigation by accident rather than reasoning.
    }
    \label{tab:conditional-mit}
\end{wraptable}



==> figs/tab-diag-mit-matrix.tex <==
\begin{wraptable}{r}{0.55\textwidth}
    \centering
    \small
    \begin{tabular}{llcccc}
        \toprule
              &     & \multicolumn{2}{c}{Noise: ✗} & \multicolumn{2}{c}{Noise: ✓} \\
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
        Agent & D   & M✗ & M✓ & M✗ & M✓ \\
        \midrule
        \multirow{2}{*}{Stratus \claude{}}
              & ✗   & 0.148 & 0.237 & 0.225 & 0.261 \\
              & ✓   & 0.067 & 0.548 & 0.113 & 0.402 \\
        % \midrule
        \multirow{2}{*}{Stratus \kimi{}}
              & ✗   & 0.261 & 0.326 & 0.316 & 0.295 \\
              & ✓   & 0.084 & 0.329 & 0.085 & 0.304 \\
        % \midrule
        \multirow{2}{*}{Claude Code}
              & ✗   & 0.126 & 0.148 & 0.148 & 0.226 \\
              & ✓   & 0.119 & 0.607 & 0.089 & 0.537 \\
        % \midrule
        \multirow{2}{*}{Codex}
              & ✗   & 0.186 & 0.114 & 0.232 & 0.175 \\
              & ✓   & 0.167 & 0.533 & 0.133 & 0.459 \\
        \bottomrule
    \end{tabular}
    \caption{Diagnosis--mitigation joint distribution. Cells show the fraction of runs falling into each outcome.}
    \label{tab:diag-mit-matrix}
    \vspace{-10pt}
\end{wraptable}


==> figs/tab-difficulty.tex <==
\begin{table}[t]
    \caption{Placeholder view for empirical difficulty. This can be instantiated either at the problem level or at the family level.}
    \label{tab:difficulty}
    \centering
    \small
    \begin{tabular}{lcccc}
        \toprule
        Problem / family & \# Runs & Diag.\ $\uparrow$ & Mit.\ $\uparrow$ & Notes \\
        \midrule
        Hard for all agents & -- & -- & -- & -- \\
        Hard to diagnose, easy to mitigate & -- & -- & -- & -- \\
        Easy to diagnose, hard to mitigate & -- & -- & -- & -- \\
        Agent-specific difficulty & -- & -- & -- & -- \\
        \bottomrule
    \end{tabular}
\end{table}


==> figs/tab-failure-modes.tex <==
\begin{table}[t]
    \caption{Manual coding of failed trajectories.}
    \label{tab:failure-modes}
    \centering
    \small
    \begin{tabular}{p{3.1cm}ccp{3.2cm}}
        \toprule
        Failure mode & Count & Share & Short description \\
        \midrule
        \bottomrule
    \end{tabular}
\end{table}


==> figs/tab-rubric-breakdown.tex <==
\begin{table}[t]
    \caption{Diagnosis rubric breakdown. $D_1$: fault localization, $D_2$: fault characterization, $D_3$: scope precision. Timeout is the fraction of runs that exceeded the time budget.}
    \label{tab:rubric-breakdown}
    \centering
    \small
    \begin{tabular}{llcccccc}
        \toprule
        Agent & Model & Noise & Diag.\ $\uparrow$ & $D_1$ & $D_2$ & $D_3$ & Timeout \% \\
        \midrule
        \multirow{4}{*}{Stratus} & \multirow{2}{*}{Claude Sonnet 4.6} & ✗ & 0.664 & 0.685 & 0.664 & 0.643 & 0.000 \\
                                 &                                    & ✓ & 0.583 & 0.583 & 0.587 & 0.577 & 0.241 \\
                                 \cmidrule{2-8}
                                 & \multirow{2}{*}{Kimi K2.5} & ✗ & 0.577 & 0.615 & 0.551 & 0.564 & 0.481 \\
                                 &                            & ✓ & 0.524 & 0.553 & 0.502 & 0.519 & 0.443 \\
        \midrule
        \multirow{2}{*}{Claude Code} & \multirow{2}{*}{Claude Sonnet 4.6} & ✗ & 0.763 & 0.792 & 0.767 & 0.730 & 0.015 \\
                                     &                                    & ✓ & 0.687 & 0.680 & 0.713 & 0.666 & 0.033 \\
        \midrule
        \multirow{2}{*}{Codex} & \multirow{2}{*}{GPT-5.4} & ✗ & 0.717 & 0.753 & 0.712 & 0.686 & 0.004 \\
                               &                                 & ✓ & 0.658 & 0.678 & 0.662 & 0.633 & 0.007 \\
        % Codex & ✗ & XX & XX & XX & XX & XX \\
        % Codex & ✓  & XX & XX & XX & XX & XX \\
        \bottomrule
    \end{tabular}
\end{table}


==> figs/tab-tool-use.tex <==
\begin{table}[t]
    \caption{Tool-use summary. This can be reported for all agents under a shared tool taxonomy or for a single agent in a focused analysis.}
    \label{tab:tool-use}
    \centering
    \small
    \begin{tabular}{lccc}
        \toprule
        Tool category & Calls & Problems touched & Share of runs \\
        \midrule
        kubectl / cluster state & -- & -- & -- \\
        Logs & -- & -- & -- \\
        Metrics & -- & -- & -- \\
        Traces / operations & -- & -- & -- \\
        App-specific tools & -- & -- & -- \\
        \bottomrule
    \end{tabular}
\end{table}

